Adaptive Retrieval Without Self-Knowledge? Bringing Uncertainty Back Home

Retrieval Augmented Generation (RAG) improves correctness of Question Answering (QA) and addresses hallucinations in Large Language Models (LLMs), yet greatly increase computational costs. Besides, RAG is not always needed as may introduce irrelevant information. Recent adaptive retrieval methods integrate LLMs' intrinsic knowledge with external information appealing to LLM self-knowledge, but they often neglect efficiency evaluations and comparisons with uncertainty estimation techniques. We bridge this gap by conducting a comprehensive analysis of 35 adaptive retrieval methods, including 8 recent approaches and 27 uncertainty estimation techniques, across 6 datasets using 10 metrics for QA performance, self-knowledge, and efficiency. Our findings show that uncertainty estimation techniques often outperform complex pipelines in terms of efficiency and self-knowledge, while maintaining comparable QA performance.

==> tables/UE_description_part2.tex <==
\begin{table*}
    \centering
    \small
    \resizebox{\textwidth}{!}{
\begin{tabular}{llllll}
\toprule
\multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method\\ acronym\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Method \\ full name\end{tabular}}}           & \multicolumn{1}{c}{\textbf{Category}}                        & \multicolumn{1}{c}{\textbf{Compute}} & \multicolumn{1}{c}{\textbf{Memory}} & \multicolumn{1}{c}{\textbf{Short description}}  
\\ \midrule

                                      
\begin{tabular}[c]{@{}l@{}}Perplexity \\ \cite{fomicheva2020unsupervised}\end{tabular}                                                                            & Perplexity                                                                                         & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score computes the average negative log\\ probability of generated tokens, which is further\\ exponentiated.
\vspace{1.1ex}

\end{tabular}                                                                                                                                                                                                                                                                                                                \\
\begin{tabular}[c]{@{}l@{}}PTrue \\ \cite{kadavath2022language}\end{tabular}                                                                                 & probability P(true)                                                                                & Reflexive                                                    & Medium                               & Low                                 & \begin{tabular}[c]{@{}l@{}}The method measures the uncertainty of the claim \\ by asking the LLM itself whether the generated claim\\ is true or not. The confidence is the probability of the\\ first generated token y1 being equal to “True”.
\vspace{1.1ex}

\end{tabular}  

\\


\begin{tabular}[c]{@{}l@{}}RDE \\ \cite{DBLP:conf/acl/YooKJK22}\end{tabular}                                                                                     & \begin{tabular}[c]{@{}l@{}}Robust density\\ estimation\end{tabular}                                & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The method improves over MD by reducing\\  the dimensionality of the last hidden state of the\\ decoder averaged over all generated tokens via PCA\\ decomposition.  Additionally, computing of the  \\ covariance matrix for each individual class is done\\ by using the Minimum Covariance Determinant\\ estimation. The uncertainty score is computed as \\ the MD in the space of reduced dimensionality.
\vspace{1.1ex}

\end{tabular}                   \\

\begin{tabular}[c]{@{}l@{}}RenyiNeg  \\ \cite{DBLP:conf/emnlp/DarrinPC23}\end{tabular}                                                                              & Rényi negentropy                                                                                   & \begin{tabular}[c]{@{}l@{}}Information-\\ based\end{tabular} & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The score computes alpha-Renyi-divergence \\ between the sample and the uniform distributions.
\vspace{1.1ex}

\end{tabular}                                                                                                                   \\
\begin{tabular}[c]{@{}l@{}}RMD  \\ \cite{DBLP:conf/iclr/0006LZKSLL23}\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Relative\\ Mahalanobis\\ distance\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}Density-\\ based\end{tabular}     & Low                                  & Low                                 & \begin{tabular}[c]{@{}l@{}}The MD distance score is adjusted by subtracting\\ from it the other  MD score computed for some\\ large general purpose dataset covering many\\ domains.
\vspace{1.1ex}

\end{tabular}                                                                                                                                                                                                        \\
\begin{tabular}[c]{@{}l@{}}SAR\\  \cite{duan2023shifting}\end{tabular}                                                                                         & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}SAR corrects generative inequalities by reviewing\\ the relevance of each token and emphasizing\\ uncertainty quantification attention to those more\\ relevant components. The relevance is measured by\\ calculating similarity of sentence before and after\\ removing the certain token.
\vspace{1.1ex}

\end{tabular}                                                                                                                                     \\
\begin{tabular}[c]{@{}l@{}}Semantic Entropy \\  \cite{DBLP:conf/iclr/KuhnGF23}\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}}Semantic\\ Entropy\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & \begin{tabular}[c]{@{}l@{}}The method aims to deal with the generated\\ sequences that have similar meaning while having\\ different probabilities according to the model. \\ The idea is to cluster generated sequences into several\\ semantically homogeneous clusters with a bi-directional\\ entailment algorithm and average the sequence\\ probabilities within the clusters.
\vspace{1.1ex}

\end{tabular}                                                                        \\
\begin{tabular}[c]{@{}l@{}}SentenceSAR\\  \cite{duan2023shifting}\end{tabular}                                                                          & \begin{tabular}[c]{@{}l@{}}Shifting Attention\\ to more Relevant \\ at Sentence level\end{tabular} & \begin{tabular}[c]{@{}l@{}}Meaning\\ diversity\end{tabular}  & High                                 & Low                                 & SAR measured at sentence-level.            
\\ \bottomrule

\end{tabular}

}
    \label{tab:ue_desc2}
    \caption{Description of the uncertainty features used in the paper.
 }

\end{table*}

==> tables/main_2hop_proxy_metrics.tex <==
% table with proxy metrics for baselines, 3 top UC, Best UC
% Correlation, ROC-AUC, Overconfidence, Undercondifence, etc from ACL paper
\begin{table*}[t]
    \centering
    \small
    \resizebox{\textwidth}{!}{

\begin{tabular}{lccccccccc}
\toprule
\multirow{2}{*}{{Method}} & \multicolumn{3}{c}{2Wiki} & \multicolumn{3}{c}{HotPot} & \multicolumn{3}{c}{Musique} \\
 & Acc & Corr & AUC & Acc & Corr & AUC & Acc & Corr & AUC \\
\midrule
AdaptiveRAG & \textbf{0.724} & \textbf{0.339} & \textbf{0.710} & 0.708 & 0.189 & 0.621 & 0.876 & 0.149 & 0.640 \\
DRAGIN & 0.682 & -0.071 & 0.456 & 0.714 & 0.011 & 0.507 & 0.894 & -0.014 & 0.487 \\
FLARE & 0.514 & 0.200 & 0.623 & 0.418 & 0.059 & 0.537 & 0.592 & 0.011 & 0.511 \\
Rowen\textsubscript{CL} & 0.316 & -0.101 & 0.459 & 0.288 & -0.134 & 0.441 & 0.108 & 0.004 & 0.503 \\
Rowen\textsubscript{CM} & 0.318 & 0.018 & 0.508 & 0.290 & -0.143 & 0.440 & 0.110 & -0.019 & 0.487 \\
Rowen\textsubscript{Hybrid} & 0.316 & -0.036 & 0.482 & 0.292 & -0.168 & 0.412 & 0.108 & -0.010 & 0.492 \\
Seakr & 0.682 & -0.217 & 0.365 & 0.714 & 0.075 & 0.548 & 0.894 & 0.065 & 0.561 \\
\midrule
EigValLaplacian & 0.688 & 0.194 & 0.620 & 0.728 & 0.266 & 0.670 & 0.894 & 0.125 & 0.617 \\
Lex-Similarity & 0.684 & 0.215 & 0.634 & \textbf{0.728} & 0.297 & {0.690} & \textbf{0.896} & 0.084 & 0.594 \\
Max Entropy & 0.688 & 0.194 & 0.621 & 0.726 & 0.295 & 0.688 & 0.894 & \textbf{0.180} & \textbf{0.669} \\
SAR & 0.686 & 0.234 & 0.645 & \textbf{0.734} & 0.303 & 0.694 & 0.894 & 0.166 & 0.660 \\
Mean Entropy & 0.684 & 0.282 & 0.675 & 0.722 & \textbf{0.310} & \textbf{0.698} & \textbf{0.896} & 0.147 & 0.637 \\

\bottomrule
\end{tabular}


}

    \caption{Caption}
    \label{tab:multi_hop_proxy}
\end{table*}


==> tables/transfer_top1UC_table.tex <==
% 6x6 table with showing top-1 UC transfer ability
